CATRE: Iterative Point Clouds Alignment for Category-level Object Pose Refinement

While category-level 9DoF object pose estimation has emerged recently, previous correspondence-based or direct regression methods are both limited in accuracy due to the huge intra-category variances in object shape and color, etc. Orthogonal to them, this work presents a category-level object pose and size refiner CATRE, which is able to iteratively enhance pose estimate from point clouds to produce accurate results. Given an initial pose estimate, CATRE predicts a relative transformation between the initial pose and ground truth by means of aligning the partially observed point cloud and an abstract shape prior. In specific, we propose a novel disentangled architecture being aware of the inherent distinctions between rotation and translation/size estimation. Extensive experiments show that our approach remarkably outperforms state-of-the-art methods on REAL275, CAMERA25, and LM benchmarks up to a speed of ~85.32Hz, and achieves competitive results on category-level tracking. We further demonstrate that CATRE can perform pose refinement on unseen category. Code and trained models are available.

==> tables/tab_new_iou.tex <==


\begin{center}
\scalebox{0.8}{
\begin{tabular}{@{}l|cc|cc|cc@{}}
    \shline
    Method & [\ncite{53}] & w/ Ours & [\ncite{46}] & w/ Ours & [\ncite{31}] & w/ Ours \\
    \hline
    \iou{50} & 47.2 & 75.4 & 68.7 & 77.0 & 74.4 & 78.6 \\
    \iou{75} & 9.4 & 41.8 & 27.0 & 44.0 & 30.8 & 44.6 \\
    \shline
\end{tabular}
}
\end{center}
